ECCentric: An Empirical Analysis of Quantum Error Correction Codes

Quantum Error Correction (QEC) is essential for building scalable quantum computers, but a lack of systematic, end-to-end evaluation methods makes it difficult to assess how different QEC codes perform under realistic conditions. The vast diversity of codes, an expansive experimental search space, and the absence of a standardized framework prevent a thorough, holistic analysis. To address this, we introduce ECCentric, an end-to-end benchmarking framework designed to systematically evaluate QEC codes across the full quantum computing stack. ECCentric is designed to be modular, extensible, and general, allowing for a comprehensive analysis of QEC code families under varying hardware topologies, noise models, and compilation strategies. Using ECCentric, we conduct the first systematic benchmarking of major QEC code families against realistic, mid-term quantum device parameters. Our empirical analysis reveals that intra-QPU execution significantly outperforms distributed methods, that qubit connectivity is a far more critical factor for reducing logical errors than increasing code distance, and that compiler overhead remains a major source of error. Furthermore, our findings suggest that trapped-ion architectures with qubit shuttling are the most promising near-term platforms and that on noisy devices, a strategic and selective application of QEC is necessary to avoid introducing more errors than are corrected. This study provides crucial, actionable insights for both hardware designers and practitioners, guiding the development of fault-tolerant quantum systems.

==> chapters/conclusions.tex <==
\section{Conclusions}
This work presents a unified benchmarking framework enabling systematic and comprehensive empirical analysis of QEC codes. Our results provide valuable insights into the performance of QEC codes under various hardware- and framework-specific limitations, contributing to the ongoing pursuit of \gls{ft} quantum hardware. Future work should investigate factors beyond the scope of this study, including the evaluation of decoders and the translation of quantum circuit gates to their \gls{ft} counterparts.

\myparagraph{Software artifact \& additional material} The evaluation code is available at [GITHUB LINK]. We present additional material in the Appendix. 



==> chapters/motivation.tex <==
\section{Motivation}
\myparagraph{Research gap} Despite the growing efforts in quantum computing benchmarking \cite{benchmarking_lorenz_2025, benchmarking_survey_proctor_2024, benchmark_qasmbench_2022, Quetschlich_2023, benchmark_supermarq_2022}, there is still no end-to-end systematic evaluation of QEC codes. Existing evaluations remain limited, typically addressing only a small selection of codes under unrealistic or artificial noise models \cite{small_codes_on_hardware_2022, comparison_shor_vs_steane_on_beacon_trappedion_2024, comparison_11codes_2009, comparison_many_codes_huang_2019}, or focusing on isolated aspects such as decoding strategies or specific hardware topologies \cite{bechmarking_controller_kurman_2024, benchmarking_ml_qec_zhao_2024, heavyhex_2025, bacon_surface_shor_trapped_ion_2020, surface_vs_realistic_noise_2014, qpandora_chatterjee_2025, steane_noise_comparison_2015, comparison_hypergraph_qldpc_2020}. Moreover, there are currently no existing benchmarking frameworks that enable such end-to-end, systematic evaluation. Existing frameworks like Stim \cite{framework_stim_2021} or Grurl et al.’s simulator \cite{framework_wille_2023} are limited to simplistic error models and do not integrate the full software stack, including compilation. As a result, current tools cannot capture how practical constraints and realistic device noise jointly impact code performance. This highlights a critical research gap: there is no comprehensive, end-to-end framework to benchmark a broad range of QEC codes under realistic noise while accounting for software stack effects and hardware constraints—an absence this work directly addresses.

\myparagraph{Challenges}
Evaluating QEC in practice is challenging. Each code exhibits distinct operational characteristics and hardware requirements. Achieving fair and informative comparisons is nontrivial: small variations in hardware assumptions, noise models, or execution details can dramatically change which code performs best. This creates a vast experimental space that is computationally demanding even with efficient simulators. Compounding the challenge, no existing framework supports testing across diverse codes under realistic device constraints.

\myparagraph{Our approach}
We address these challenges by proposing a framework designed to be efficient, systematic, and extensible. It combines stabilizer-based simulation with detailed noise and full compilation stacks to capture realistic overheads, enforces consistent pipelines so differences reflect the codes themselves rather than artifacts of modeling or execution, and provides a modular design that supports a wide range of codes, architectures, and compilers while remaining adaptable to future developments. By linking theoretical code properties to real-device performance, our work delivers a practical, hardware-aware tool to guide the path toward fault-tolerant quantum computing.


==> figures/axes.tex <==
\begin{tikzpicture}
    \draw (0,0) -- (4,0) -- (2,3.464) -- cycle;
    
    \node[above] at (2,3.464) {Noise Model};
    \node[below left] at (0,0) {Hardware};
    \node[below right] at (4,0) {Framework};
    
    \node at (2,1.2) {ECCentric};
    
\end{tikzpicture}

==> figures/setup_general.tex <==
 \begin{tikzpicture}[node distance=2.3cm, auto]
         \node (Ecc) [draw,text width=11.4cm, minimum height=3cm, text depth = 2.5cm, align=center, fill=yellow!25] at (4.65, 0.5) {\textbf{ECCentric}};
        \node (A) [draw, rectangle, minimum width=2cm, minimum height=1.5cm, align=center, fill=orange!20] {Encoded\\Quantum\\Memory};
        \node (B) [draw, rectangle, minimum width=2cm, minimum height=1.5cm, right of=A, align=center, fill=orange!20] {Transpilation};
        \node (D) [draw, rectangle, minimum width=2cm, minimum height=1.5cm, right of=B, align=center, fill=orange!20] {Noise\\Addition};
        \node (E) [draw, rectangle, minimum width=2cm, minimum height=1.5cm, right of=D, align=center, fill=orange!20] {Stabilizer\\Simulation};
        \node (F) [draw, rectangle, minimum width=2cm, minimum height=1.5cm, right of=E, align=center, fill=orange!20] {Measurement\\and\\Correction};
        \node (G) [draw, rectangle, minimum width=1.5cm, minimum height=1.5cm, right of=F, align=center, fill=gray!20] {Logical\\Error\\Rate};
        \node (Q) [draw,text width=4.15cm, minimum height=0.55cm, align=center, fill=blue!20] at (1.18, 1.15) {Qiskit};
        \node (S) [draw,text width=6.46cm, minimum height=0.55cm, align=center, fill=purple!20] at (6.96, 1.15) {Stim};


        \draw[->] (A) -- (B);
        \draw[->] (B) -- (D);
        \draw[->] (D) -- (E);
        \draw[->] (E) -- (F);
        \draw[->] (F) -- (G);
        \draw[dotted] (3.49,-0.75) -- (3.49,1.5);
        
        
        
        
\end{tikzpicture}

==> figures/steane_small.tex <==
\begin{tikzpicture}[scale=1]
  \coordinate (A) at (1,2);
  \coordinate (B) at (1.5,1);
  \coordinate (C) at (1,0.66);
  \coordinate (D) at (0.5,1);
  \coordinate (E) at (0,0);
  \coordinate (F) at (1,0);
  \coordinate (G) at (2,0);

  \fill[red!30,opacity=0.5] 
    (A) -- (B) -- (C) -- (D) -- cycle;
  \fill[green!30,opacity=0.5] 
    (C) -- (D) -- (E) -- (F) -- cycle;
  \fill[blue!30,opacity=0.5] 
    (C) -- (B) -- (G) -- (F) -- cycle;

  \draw[thick] (A) -- (B) -- (C) -- (D) -- cycle;
  \draw[thick] (D) -- (E) -- (F) -- (C);
  \draw[thick] (F) -- (G) -- (B) -- (C) -- cycle;

  \foreach \P in {A,B,C,D,E,F,G}{
    \filldraw[fill=white,draw=black] (\P) circle[radius=3pt];
  }
\end{tikzpicture}

==> figures/surface_code.tex <==
\begin{tikzpicture}[scale=1]

  \foreach \x in {0,...,3} {
    \foreach \y in {0,...,2} {
      \pgfmathtruncatemacro{\modval}{mod(\x+\y,2)}
      \ifnum\modval=0
        \fill[blue!30,opacity=0.5] (\x,\y) rectangle ++(1,1);
      \else
        \fill[orange!30,opacity=0.5] (\x,\y) rectangle ++(1,1);
      \fi
    }
  }

    \fill[red!30]   (0,0) rectangle ++(1,1);
    \fill[green!30]   (2,1) rectangle ++(1,1);


    \fill[fill=orange!30,opacity=0.5] (0,3) arc (180:0:0.5) -- cycle;
    \fill[fill=orange!30,opacity=0.5] (2,3) arc (180:0:0.5) -- cycle;

   \fill[fill=orange!30,opacity=0.5] (0,0) arc (180:360:0.5) -- cycle;
   \fill[fill=orange!30,opacity=0.5] (2,0) arc (180:360:0.5) -- cycle;

   \fill[fill=orange!30,opacity=0.5] (0,3) arc (180:0:0.5) -- cycle;
    \fill[fill=orange!30,opacity=0.5] (2,3) arc (180:0:0.5) -- cycle;

   \fill[fill=blue!30,opacity=0.5] (0,1) arc (270:90:0.5) -- cycle;
   \fill[fill=blue!30,opacity=0.5] (4,0) arc (270:450:0.5) -- cycle;
   \fill[fill=blue!30,opacity=0.5] (4,2) arc (270:450:0.5) -- cycle;

  \foreach \y in {0,...,3} {
    \draw[thick] (0,\y) -- (4,\y);
  }
  \foreach \x in {0,...,4} {
    \draw[thick] (\x,0) -- (\x,3);
  }

  \foreach \x in {0,...,4} {
    \foreach \y in {0,...,3} {
      \draw[fill=white,draw=black] (\x,\y) circle[radius=2pt];
    }
  }

\end{tikzpicture}

==> figures/taxonomy_venn.tex <==
\newcommand{\boundellipse}[3]{(#1) ellipse (#2 and #3);}
\begin{tikzpicture}
\def\radius{2cm}
\colorlet{subsystem}{blue!70}
\colorlet{stabilizer}{red!70}
\colorlet{topological}{green!70}
\colorlet{concatenated}{cyan!70}
\colorlet{ldpc}{orange!70}

\coordinate (subs) at (0,1.2);
\coordinate (stabilizer) at (0, 0.65);
\coordinate (topo) at (1.2,-0.3);
\coordinate (ldpc) at (-1.2,-0.3);
\coordinate (concat) at (0, -1.2);

\draw[fill=subsystem, fill opacity=0.5] \boundellipse{0,-0.3}{3.6\radius}{1.8\radius};
\draw[fill=stabilizer, fill opacity=0.5] \boundellipse{0,-0.5}{3.0\radius}{1.5\radius};
\draw[fill=topological, fill opacity=0.5] \boundellipse{1.2,-0.3}{1.4\radius}{0.7\radius};
\draw[fill=ldpc, fill opacity=0.5] \boundellipse{-1.2,-0.3}{1.4\radius}{0.7\radius};
\draw[fill=concatenated, fill opacity=0.5] \boundellipse{0,-1.2}{1.4\radius}{0.7\radius};

\node at (subs) {Subsystem};
\node at (stabilizer) {Stabilizer};
\node at (topo) {Topological};
\node at (concat) {Concatenated};
\node at (ldpc) {LDPC};

\end{tikzpicture}

==> figures_tex/scope_spiderchart.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \scalebox{0.65}{
        \newcommand{\D}{7}
        \newcommand{\U}{7}
        
        \newdimen\R
        \R=3.5cm 
        \newdimen\L
        \L=4cm
        
        \newcommand{\A}{360/\D}
        
        \begin{tikzpicture}[scale=0.8]
          \path (0:0cm) coordinate (O);
        
          \foreach \X in {1,...,\D}{
            \draw (\X*\A:0) -- (\X*\A:\R);
          }
        
          \foreach \Y in {0,...,\U}{
            \foreach \X in {1,...,\D}{
              \path (\X*\A:\Y*\R/\U) coordinate (D\X-\Y);
              \fill (D\X-\Y) circle (1pt);
            }
            \draw [opacity=0.3] (0:\Y*\R/\U) \foreach \X in {1,...,\D}{
                -- (\X*\A:\Y*\R/\U)
            } -- cycle;
          }
        
          \path (1*\A:\L) node (L1) {\normalsize Codes};
          \path (2*\A:\L) node (L2) {\normalsize Topology};
          \path (3*\A:\L) node[xshift=-3mm] (L3) {\normalsize FT Gates};
          \path (4*\A:\L) node[xshift=-3mm] (L4) {\normalsize Decoders};
          \path (5*\A:\L) node (L5) {\normalsize Noise Model};
          \path (6*\A:\L) node (L6) {\normalsize Translation};
          \path (7*\A:\L) node[xshift=3mm] (L7) {\normalsize Mapping};

        
          \draw [color=blue,line width=1.5pt,opacity=0.5,fill=blue, fill opacity=0.25]
            (D1-6) --
            (D2-6) --
            (D3-1) --
            (D4-2) --
            (D5-7) --
            (D6-5) --
            (D7-5) -- cycle;
        
        \end{tikzpicture}
        
    }
    \caption{Coverage of problem dimensions addressed in this project. \aleksandra{TODO: update}}
    \label{fig:axes}
\end{wrapfigure}


==> plots/eval_dqc/flamingo.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45]{plots/eval_dqc/dqc_Flamingo.pdf}
    \vspace{-5pt}
    \caption{Performance of QEC codes on a single QPU vs. on the entire DQC architecture of IBM Flamingo. {\em a) With original IBM Flamingo noise. b) With noise downscaled tenfold.}}
    \label{fig:dqc}
\end{figure}

==> plots/eval_dqc/nighthawk.tex <==
\begin{figure}[t]
    \centering
     \includegraphics[scale=0.45]{plots/eval_dqc/dqc_Nighthawk.pdf}
     \vspace{-5pt}
    \caption{Performance of QEC codes on a single QPU vs. on the entire DQC architecture of IBM Nighthawk. {\em a) With original IBM Flamingo noise. b) With noise downscaled tenfold.}}
    \label{fig:dqc_ext}
\end{figure}

==> plots/eval_size/size.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
 \includegraphics[scale=0.45]{plots/eval_size/size_SI1000_0.004.pdf}
    \caption{Logical error rates of different QEC codes at maximal available code distance across backend sizes under the SI1000 noise model. {\em Highlighted points mark an increase in the maximal achievable code distance.}}
    \label{fig:size}
\end{wrapfigure}


==> plots/eval_translating/gate_base.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_h2_base.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_ibm_heron_base.pdf}
    \end{subfigure}
    \caption{Gate overhead introduced during translating to H2 and IBM Heron gate sets using unoptimized TKET and Qiskit. \aleksandra{WIP: I need to decide how to connect the plots in common flow, fix colors and spaces to look better and not-repetitive. Main points: different translators make huge difference (TKET vs Qiskit), different codes may have different normalized overheads which is weird, optimized TKET and Qiskit make difference but not that much.}}
    \label{fig:translating_base}
\end{figure}

==> plots/eval_translating/gate_base_norm.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_norm_h2_base.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_norm_ibm_heron_base.pdf}
    \end{subfigure}
    \caption{Normalized gate overhead introduced during translating to H2 and IBM Heron gate sets using unoptimized TKET and Qiskit.}
    \label{fig:translating_base_norm}
\end{figure}

==> plots/eval_translating/gate_opt.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_h2_optimized.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_ibm_heron_optimized.pdf}
    \end{subfigure}
    \caption{Gate overhead introduced during translating to H2 and IBM Heron gate sets using optimized TKET and Qiskit.}
    \label{fig:translating_opt}
\end{figure}

==> plots/eval_translating/gate_opt_norm.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_norm_h2_optimized.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.4]{plots/eval_translating/gate_overhead_norm_ibm_heron_optimized.pdf}
    \end{subfigure}
    \caption{Normalized gate overhead introduced during translating to H2 and IBM Heron gate sets using optimized TKET and Qiskit.}
    \label{fig:translating_base}
\end{figure}

==> plots/eval_translating/gate_overhead_norm.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45]{plots/eval_translating/gate_overhead_normalized.pdf}
    \caption{Normalized gate overhead when converting to IBM Heron and Quantinuum H2 gate sets using TKET and Qiskit.}
    \label{fig:translating_norm}
\end{figure}

==> tables/accumulated_errors.tex <==

\begin{table}[t]
\centering

\caption{Logical error rates for an unprotected qubit and for different codes with uncorrected and corrected protection over the same number of cycles at various error probabilities.}

\fontsize{8}{9}\selectfont{
\begin{tabular}{|c|c|cccccc|}
\hline
\textbf{Err. Prob.} & \textbf{Type} & Surface & Gross & Heavy-hex & Con. Steane & Color & Bacon-Shor \\
\hline
\multirow{2}{*}{0.004} & Without QEC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
                       & With QEC   & \textbf{0.000} & \textbf{0.000} & 0.003 & 0.044 & \textbf{0.000} & 0.106 \\
\hline
\multirow{2}{*}{0.006} & Without QEC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
                       & With QEC    & 0.001 & 0.001 & 0.045 & 0.065 & 0.002 & 0.301 \\
\hline
\multirow{2}{*}{0.008} & Without QEC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
                       & With QEC    & 0.002 & 0.005 & 0.162 & 0.098 & 0.006 & 0.367 \\
\hline
\end{tabular}
}
\label{tab:wqec_qec}
\end{table}


==> tables/changes.tex <==
\fontsize{8}{9}\selectfont
\begin{longtable}{|p{0.5cm}|p{5.5cm}|p{5.5cm}|p{0.8cm}|}
\hline
\textbf{ID} & \textbf{Comment} & \textbf{How do we plan to address the comment?} & \textbf{Section} \\
\hline
\endfirsthead

\hline
\textbf{ID} & \textbf{Comment} & \textbf{How do we plan to address the comment?} & \textbf{Section} \\
\hline
\endhead
\rowcolor{blue!15}

C1 &
\textit{Figure 9 is hard to interpret. It is unclear what the highlighted points mean, ``Log.'' as an abbreviation for ``Logical'' rather than ``Logarithmic'' is confusing, and the paper claims that this figure answers RQ1 about code distance, but the compared distances are unclear.} &
We replace ``Log.'' with ``Logical'' on the plots to improve clarity. In the caption of Fig.~9 we clarify that the mark on the line of each code represents the distance change. &
\makecell[l]{\S4--6} \\
\hline
\rowcolor{blue!15}
C2 &
\textit{In Figure 10, error bars should be shown around the 0-error empirical measurement, and the y-axis extending to $10^{-6}$ is misleading given 1000 shots.} &
In Fig.~10 we modify the y-axis so that error bars at 0 errors are visible and present $0.001$ as the minimal observable error rate. &
\makecell[l]{\S4} \\
\hline
\rowcolor{blue!15}
C3 &
\textit{Figure 25b may be missing the ``o'' in ``w/o Decoding'', and Fig.~25c should use standard notation (500) instead of scientific notation (5e2).} &
We add the missing ``o'' in ``w/o Decoding'' in Fig.~25b and replace the scientific notation in Fig.~25c with the standard form. &
\makecell[l]{\S6} \\
\hline
\rowcolor{yellow!15}
O1 &
\textit{Plots and results previously moved to the appendix due to space limitations should be returned to the main paper.} &
We restore plots and results previously moved to the appendix to the main paper. &
\makecell[l]{\S4--6} \\
\hline

\end{longtable}
\normalsize

==> tables/combinations.tex <==
\begin{table}[h!]
\caption{Summary of the study dimensions.}
\centering
\fontsize{8}{9}\selectfont
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{QEC Codes} & \textbf{Noise Models} & \textbf{Topologies} & \textbf{Translation} & \textbf{Mapping} & \textbf{Routing} \\ \hline
Surface code & Artificial Constant & Artificial grid & TKET & Trivial & Basic \\
Color code & Artificial SI1000 & Artificial cube & Qiskit & Dense & Stochastic \\
Gross code & Q. Apollo & Artificial fully-connected & Qiskit optimized & Sabre & Sabre \\
Bacon-Shor code & Infleqtion & Q. Apollo & BQskit* &  &  \\
Heavy-hex code & Google Willow & Infleqtion &  &  &  \\
Con. Steane code & IBM Flamingo & Google Willow &  &  &  \\
 &  & IBM Flamingo &  &  &  \\
\end{tabular}
\label{tab:study_summary}
\end{table}


==> tables/device_error_rates.tex <==
\begin{table}[h!]
\centering
\fontsize{8}{9}\selectfont
\caption{Error rates of different quantum devices and an artificial noise model. 
{\em Quantinuum (Q.) Apollo~\cite{Quantinuum2024Roadmap} data are extrapolated from H2 device specifications \cite{QuantinuumHardwareSpecs}. For Infleqtion, reset error is included in readout error, leakage in gate error, and SPAM is approximated as measurement plus reset, as it is not directly reported~\cite{radnaev2025universalneutralatomquantumcomputer}.}}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & Neutral Atom & Trapped-Ion & \multicolumn{2}{c|}{Superconducting} & Artificial \\
\hline
 & \makecell{Infleqtion \cite{radnaev2025universalneutralatomquantumcomputer}} & \makecell{Q. Apollo \cite{QuantinuumHardwareSpecs, Quantinuum2024Roadmap}} & \makecell{Willow \cite{Willow2025}} & \makecell{Flamingo \cite{AbuGhanem_2025}} & \makecell{SI1000 \cite{comparison_honeycomb_vs_surface_2021}} \\
\hline
SQ & $9.8\times10^{-4}$ & $8.0\times10^{-6}$ & $6.2\times10^{-4}$ & $2.5\times10^{-4}$ & $p/10$ \\
\hline
2Q & $6.5\times10^{-3}$ & $1.4\times10^{-4}$ & $2.8\times10^{-3}$ & $2.0\times10^{-3}$ & $p$ \\
\hline
SPAM & $4.0\times10^{-3}$ & $1.33\times10^{-4}$ & $9.5\times10^{-3}$ & $2.5\times10^{-4}$ & $2p+5p$ \\
\hline
Idle & - & $5.3\times10^{-5}$ & $9.0\times10^{-3}$ & - & $p/10$ \\
\hline
Crosstalk & - & $6.3\times10^{-7}$ & $5.5\times10^{-4}$ & - & $0$ \\
\hline
Leakage & - & $4.3\times10^{-5}$ & $2.5\times10^{-4}$ & - & $0$ \\
\hline
T1 [s] & $2.6\times10^{1}$ & $>6.0\times10^{1}$ & $6.8\times10^{-5}$ & $1.9\times10^{-4}$ & $0$ \\
\hline
T2 [s] & $2.8\times10^{0}$ & $\sim4.0\times10^{0}$ & $8.9\times10^{-5}$ & $1.3\times10^{-4}$ & $0$ \\
\hline
\end{tabular}
\label{tab:error_rates}
\end{table}


==> tables/findings_summary.tex <==
\begin{table}[h!]
\caption{Summary of the key findings of this work and their corresponding implications.}
\centering
\begin{tabular}{|p{6.5cm}|p{6.5cm}|}
\hline
\textbf{Our key findings} & \textbf{Implications} \\
\hline
Quantinuum’s Apollo architecture enables full error suppression; even a tenfold reduction of Flamingo’s current error rates would already make effective error correction feasible. 
& Based on current industry roadmaps, the realization of fully functional quantum error correction appears achievable within the next five years. \\
\hline
Restricting code size to a single QPU yields 58.8\% lower logical error than extending across the maximum distance possible on a DQC device. 
& On \gls{dqc} platforms, code patches should be confined to a single, non-distributed QPU to achieve optimal performance. \\
\hline
The code introduces logical errors at lower error probabilities than would naturally occur in unprotected quantum memory. \aleksandra{SI 1000 0.006 -- no code works, 0.004 -- only half}
& In environments with very low idle-error rates, unprotected quantum memory may provide more reliable storage than memory protected by error-correcting codes. \\
\hline
Variations in qubit quality are largely irrelevant when using \gls{qec}, provided the average qubit quality remains constant. 
& When employing \gls{qec}, compilation strategies tailored to individual qubit quality may be unnecessary, or only beneficial in a limited scope. \\
\hline
\end{tabular}
\label{tab:findings}
\end{table}


==> tables/google_noise_models.tex <==
\begin{table}[h!]
\centering
\caption{Noise models proposed by Gidney et al.~\cite{comparison_honeycomb_vs_surface_2021}.}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
 & SQ & 2Q & Readout & Reset & Idle \\
\hline
SD6 & 0 & 0 & 0 & 0 & 0 \\
\hline
EM3 & 0 & 0 & 0 & 0 & 0 \\
\hline
SI1000 & 0 & 0 & 0 & 0 & 0 \\
\hline
\end{tabular}
\label{tab:noise_models}
\end{table}


==> tables/revisions.tex <==
\fontsize{8}{9}\selectfont
\begin{longtable}{|p{0.5cm}|p{5cm}|p{5cm}|p{0.7cm}|p{1cm}|}
\hline
\textbf{ID} & \textbf{Comment} & \textbf{Revision summary} & \textbf{Section} & \textbf{New~exp.} \\
\hline
\endfirsthead

\hline
\textbf{ID} & \textbf{Comment} & \textbf{Revision summary} & \textbf{Section} & \textbf{New~exp.} \\
\hline
\endhead
\rowcolor{blue!15}

M1.1 &
\textit{Describe what exactly is simulated (circuits, code distances, operations).} &
We update \S3.3 to specify our methodology: stabilizer-based simulations of quantum circuits representing a quantum memory encoded using the maximum code distance supported by the topology. We also clarified that fault-tolerant logical operations are excluded.
&
\makecell[l]{\S3.3} & No. \\
\rowcolor{blue!15}
M1.2 &
\textit{How large-scale experiments are made tractable, what approximations are used?} &  We clarify in \S3.3 that simulations are exact and use no approximations. The memory resources required to make these large-scale instances tractable are now detailed in the new \S7.
&
\makecell[l]{\S3.3\\\S7} & No. \\
\rowcolor{blue!15}
M1.3 &
\textit{Are 1000 shots sufficient for reliable logical error estimation?} & We clarify in \S3.3 that while 1000 shots do not yield high precision, they provide confidence intervals tight enough to differentiate practical low-error regimes from code failure
&
\makecell[l]{\S3.3} & No. \\
\rowcolor{blue!15}
M2 &
\textit{Clarify the impact of excluding fault-tolerant gate constructions and classical decoder latency.} & We exclude FT gate constructions because the only existing framework supports the surface code and remains limited and under active development. Developing a general, scalable FT gate constructor would itself constitute a substantial standalone contribution. We also omit classical decoder latency, as it depends strongly on the code, decoder, and hardware platform, making any fixed latency assumption unsuitable for a general comparative analysis. We expand s3.1 to clarify these exclusions and discuss their impact.
&
\makecell[l]{\S3.1\\\S7}  &  No. \\
\rowcolor{blue!15}
M3 &
\textit{Provide all noise sources, expand heterogeneity, add a no-variance baseline, and justify claims that heterogeneity is negligible.} & We provide the noise sources in \S2 and in \S3.3, we state every available noise source for simulation. We extend \S4.3 to include a no-variance baseline and to account for readout error as an additional source of variation.
&
\makecell[l]{\S2\\\S3.3\\\S4.3}  & Yes. \\
\rowcolor{blue!15}
M4.1 &
\textit{Clarify the claim that heterogeneity does not matter with the finding that QEC can be harmful at certain physical error rates.} & 
In \S6.2, we now add a sentence emphasizing that our goal is to observe the growth rate of the logical error rate for protected and unprotected circuits across different average error probabilities, illustrating how quickly the codes become detrimental once their threshold is exceeded.
&
\makecell[l]{\S6.2}  & No. \\
\rowcolor{blue!15}
M4.2 &
\textit{Where QEC helps vs. hurts, show how thresholds depend on topology/noise, and provide concrete guidance on selective deployment of QEC.} & We extend the experiments of \S6.2 by adding a plot showing the thresholds of the codes in a realistic setup, allowing us to precisely identify the regimes where the codes become harmful. We discuss how the threshold would change with the imposition of additional limitations (e.g., limited topology). We make the takeaway more explicit regarding the selective deployment of QEC.
&
\makecell[l]{\S6.2}  &  Yes. \\
\rowcolor{blue!15}
M5.1 &
\textit{Provide decoder configurations and runtime costs.} & We provide a more detailed description of each experimental configuration and include a runtime analysis of the decoder in \S6.2.
&
\makecell[l]{\S4--6}  & Yes \\
\rowcolor{blue!15}
M5.2 &
\textit{Characterize ECCentric’s runtime/memory scaling and feasibility limits.} & We add a new Section \S7 (Limitations) to discuss and analyze the runtime of ECCentric, as well as its memory usage and limits. In \S7, we also provide results showing runtime and memory consumption for different sizes of experiments.
&
\makecell[l]{\S7}  & Yes. \\
\rowcolor{blue!15}
M5.3 &
\textit{Clarify wording of results.} & We reword our observations in a more precise way (e.g., we replace "zero logical error" with "no errors observed").
&
\makecell[l]{\S4--6}  & No. \\

\hline
\rowcolor{red!15}
A1 &
\textit{Simulation setup (number of shots, executed circuits).} & See M.1.1-M.1.3.
&
\makecell[l]{\S3.3}  & No. \\
\rowcolor{red!15}
A2 &
\textit{FT gates and classical technologies appear in figures but are not covered in the study.} & See M2.
&
\makecell[l]{\S3.1\\\S7}  &  No. \\
\rowcolor{red!15}
A3 &
\textit{Variance section lacks a no-variance baseline and broader variation.} & See M.3.
&
\makecell[l]{\S4.3}  & Yes.  \\
\rowcolor{red!15}
A4 &
\textit{Connectivity recommendations should consider near-term architectures.} &
We extend \S4.2 to frame full connectivity as an idealized upper bound and discuss realistic partial-connectivity options, including shuttling.
&
\makecell[l]{\S4.2}  & No. \\
\rowcolor{red!15}
A5.1 &
\textit{Contradiction between takeaways: heterogeneity vs.\ QEC being counterproductive.} & See M4.1.
&
\makecell[l]{\S4.3}  & No. \\
\rowcolor{red!15}
A5.2 &
\textit{QEC isn't always beneficial; define thresholds and propose selective deployment.} & See M4.2.
&
\makecell[l]{\S6.2}  & Yes. \\
\rowcolor{red!15}
A6.1 &
\textit{Decoder section is underspecified.} & We provide the decoder settings used in \S6.1 and discuss how these settings affect runtime and accuracy.
&
\makecell[l]{\S6.1}  & No. \\
\rowcolor{red!15}
A6.2 &
\textit{Wording is misleading.} & See M5.3.
&
\makecell[l]{\S4--6}  & No. \\

\hline
\rowcolor{green!15}
B1 &
\textit{No experimental validation on real hardware.} &
We add a plot showing errors in a quantum memory circuit run on an actual device (e.g., IBM Heron), with a widely used error model and with our own model. 
&
\makecell[l]{\S3.3} &  Yes. \\
\rowcolor{green!15}
B2 &
\textit{All experiments are memory-only, not full logical circuits.} & See M2.
&
\makecell[l]{\S3.1\\\S7}  &  No. \\
\rowcolor{green!15}
B3 &
\textit{ECCentric runtime and memory scaling are not quantified.} & See M5.2.
&
\makecell[l]{\S7}  &  Yes. \\

\hline
\rowcolor{yellow!15}
C1 &
\textit{Limitations of ECCentric.} & See M2 and M5.2.
&
\makecell[l]{\S3.1\\\S7}  &  No. \\
\rowcolor{yellow!15}
C2 &
\textit{Itemize contributions.} & We replace the last paragraph of \S1 with contribution formatted as a list.
&
\makecell[l]{\S1}  & No. \\
\hline
\rowcolor{cyan!15}
O1 &
\textit{Qiskit-qec should be removed.} & We remove the sentence about qiskit-qec from \S3.3. We update the experiments whose results change by this change. 
&
\makecell[l]{\S3.3\\\S4-6}  &  Yes. \\
\rowcolor{cyan!15}
O2 &
\textit{Minor improvements.} & We make all necessary minor corrections in the paper.
&
\makecell[l]{\S1-10}  & No. \\
\rowcolor{cyan!15}
O3 &
\textit{Selected plots and results need to be moved to the appendix.} & We move the less important results to the appendix for space consideration.
&
\makecell[l]{\S4-6}  & No. \\


\hline
\end{longtable}
\normalsize


==> tables/scope_coverage_minimal.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{RQ} & \textbf{Codes} & \textbf{Topologies} & \textbf{Devices} & \textbf{Noise} & \textbf{Compilation} \\
\hline
\textbf{Q1: sec. \ref{sec:hardware}} & \cmark & \cmark & \xmark & \cmark & \xmark \\
\hline
\textbf{Q2: sec. \ref{sec:hardware}} & \cmark & \cmark & \xmark & \cmark & \xmark \\
\hline
\textbf{Q3: sec. \ref{sec:hardware}} & \cmark & \cmark & \xmark & \cmark & \xmark \\
\hline
\textbf{Q4: sec. \ref{sec:hardware}} & \cmark & \xmark & \cmark & \cmark & \xmark \\
\hline
\textbf{Q5: sec. \ref{sec:hardware}} & \cmark & \xmark & \cmark & \xmark & \cmark \\
\hline
\textbf{Q6: sec. \ref{sec:hardware}} & \cmark & \xmark & \cmark & \cmark & \xmark \\
\hline
\textbf{Q7: sec. \ref{sec:hardware}} & \cmark & \xmark & \cmark & \cmark & \xmark \\
\hline
\textbf{Q8: sec. \ref{sec:hardware}} & \cmark & \xmark & \cmark & \cmark & \xmark \\
\hline
\textbf{Q9: sec. \ref{sec:hardware}} & \cmark & \xmark & \cmark & \cmark & \xmark \\
\hline
\textbf{Q10: sec. \ref{sec:hardware}} & \cmark & \xmark & \cmark & \cmark & \xmark \\
\hline
\end{tabular}


==> tables/scope_coverage_old.tex <==
\begin{table}[htbp]
\centering

\caption{Research questions we pursue in this work and their relations to the considered problem dimensions. \aleksandra{Update according to the new questions.}}
{
\fontsize{8}{9}\selectfont
\begin{tabular}{|>{\raggedright\arraybackslash}p{6cm}|c|c|c|c|c|}
\hline
\makecell[c]{\textbf{Research Question}} & \textbf{Codes} & \textbf{Topologies} & \textbf{Noise} & \textbf{Mapping} & \textbf{Translation} \\
\hline
How does topology size influence the effectiveness of the chosen \gls{qec} codes? & \cmark & \cmark & \cmark & \cmark & \xmark \\
\hline
How does topology connectivity influence the effectiveness of the chosen \gls{qec} codes? & \cmark & \cmark & \cmark & \cmark & \xmark \\
\hline
How effective are the chosen \gls{qec} codes on realistic mid-term topologies? & \cmark & \cmark & \xmark & \cmark & \xmark \\
\hline
How does the variance of qubit error probabilities influence the \gls{qec} codes' effectiveness? & \cmark & \xmark & \cmark & \cmark & \xmark \\
\hline
How effective are \gls{qec} codes on distributed QPUs? & \cmark & \cmark & \xmark & \cmark & \xmark \\
\hline
How effective are the chosen \gls{qec} codes on different quantum technologies? & \cmark & \xmark & \cmark & \xmark & \xmark \\
\hline
How does mapping and routing influence error probabilities? & \xmark & \cmark & \xmark & \cmark & \xmark \\
\hline
How does translation to the backend’s basis set influence error probabilities? & \cmark & \xmark & \xmark & \xmark & \cmark \\
\hline
How do the error rates of the devices correspond to the required error thresholds of \gls{qec} codes & \cmark & \xmark & \cmark & \xmark & \xmark \\
\hline
To what extent do chosen \gls{qec} codes accumulate additional errors? & \cmark & \xmark & \cmark & \cmark & \cmark \\
\hline
\end{tabular}
}

\label{tab:research_questions}
\end{table}


==> tables/study_summary.tex <==
\begin{table}[t]
\caption{Summary of the study dimensions. \aleksandra{TBD}}
\centering
\fontsize{8}{9}\selectfont
\begin{tabular}{|p{3cm}|p{2.7cm}|p{2.7cm}|p{2.7cm}|}
\hline
\textbf{QEC Codes} & \textbf{QPU Noise Models} & \textbf{QPU Topologies} & \textbf{Compilation} \\ \hline
\makecell[l]{Selection of representative\\ codes from major \gls{qec}\\families} &
\makecell[l]{Artificial noise models\\ and noise models from\\4 mid-term quantum\\devices} &
\makecell[l]{Artificial topologies \\varying in size an\\connectivity, and 4\\real-device topologies} &
\makecell[l]{Different compilers,\\ different mapping and\\routing  heuristics} \\ \hline
\end{tabular}
\label{tab:study_summary}
\end{table}
